Continual Vision-based Reinforcement Learning with Group Symmetries

Continual reinforcement learning aims to sequentially learn a variety of tasks, retaining the ability to perform previously encountered tasks while simultaneously developing new policies for novel tasks. However, current continual RL approaches overlook the fact that certain tasks are identical under basic group operations like rotations or translations, especially with visual inputs. They may unnecessarily learn and maintain a new policy for each similar task, leading to poor sample efficiency and weak generalization capability. To address this, we introduce a unique Continual Vision-based Reinforcement Learning method that recognizes Group Symmetries, called COVERS, cultivating a policy for each group of equivalent tasks rather than individual tasks. COVERS employs a proximal policy optimization-based RL algorithm with an equivariant feature extractor and a novel task grouping mechanism that relies on the extracted invariant features. We evaluate COVERS on sequences of table-top manipulation tasks that incorporate image observations and robot proprioceptive information in both simulations and on real robot platforms. Our results show that COVERS accurately assigns tasks to their respective groups and significantly outperforms existing methods in terms of generalization capability.

==> contents/pseudo_code.tex <==
\begin{algorithm}[t]
\caption{Continual RL with Group Symmetries}
\label{alg:main}
\textbf{Input}: Wasserstein distance threshold $d_{\epsilon}$, initial frame number$k$ \\
\textbf{Output}: collection of policies $\Pi$ \\
\textbf{Initialization}: $\Pi \leftarrow \{\emptyset\}, K \leftarrow 0$ \\
\vspace{-0.1in}

\begin{algorithmic}[1] %[1] enables line numbers
\WHILE{\emph{task not finish}}
% Empty the state buffer D
\STATE $O \leftarrow \emptyset$
% Roll-out N episode in the environment with the current policy
\FOR{$i = 1, 2, \ldots, N$}
\STATE $j \leftarrow 0$
\WHILE{\emph{episode not finish}}
\STATE $a_{t} \sim \pi_{\theta}(s_{t}|a_{t})$
\STATE $s_{t+1} \sim p(s_{t+1}|s_{t},a_{t})$
\IF{$j < k$}
\STATE $O \leftarrow O \cup \{s(t)\}$
\ENDIF
\STATE $j \leftarrow j + 1$
\ENDWHILE
\ENDFOR
% compute the distance to each policy
\STATE $D \leftarrow \emptyset$
\FORALL{$\pi_{i} \in \Pi$}
\STATE $q_{i, O} = f_i(O)$
\STATE $q_{i, B_i} = f_i(B_i)$
\STATE $d_{i} = W(q_{i, O}, q_{i, B_i})$
\STATE $D \leftarrow D \cup \{d_{i}\}$
\ENDFOR
% Change current policy
\STATE $j \leftarrow arg min D$
\IF{$d_j > d_{\epsilon}$}
% Create new policy
\STATE Initialize a new policy $\pi_{\theta}$
\STATE $\Pi \leftarrow \Pi \cup \{\pi_{\theta}\}$
\ELSE
\STATE $\pi_{\theta} \leftarrow \pi_{j}$
\ENDIF
% % \STATE Reset environment
% \STATE Get current observation $s_t$
% \FORALL{policy $\pi_{\theta_k} \in \Pi$}
% \STATE Compute Mahalanobis distance $d_k$ to policy $\pi_{\theta_k}$
% \ENDFOR
% \STATE Get policy $\pi_{\theta^{*}}$ with minimal distance $d^{*}$
% \IF{$d^{*} > d_{\epsilon}$}
% \STATE Initialize a new policy $\pi_{\theta_K}$ and its buffer $\mathcal{B}_K = \{ \emptyset \}$
% \STATE $\Pi \leftarrow \Pi \cup \{\pi_{\theta_K}\}$, $K \leftarrow K+1$
% \STATE $\pi_{\theta} \leftarrow \pi_{\theta_K}$, $\mathcal{B} \leftarrow \mathcal{B}_K$
% \ELSE
% \STATE $\pi_{\theta} \leftarrow \pi_{\theta^{*}}$, $\mathcal{B} \leftarrow \mathcal{B}^*$
% \ENDIF
% \REPEAT
% \STATE Sample action $a \sim \pi_{\theta}(\cdot | s_t)$ 
% % \STATE take action $a$, observe $r_t, s_{t+1}$
% \STATE Update state buffer
% $\mathcal{B} \leftarrow \mathcal{B} \cup \{s_t\}$
% \UNTIL{episode finish}

\STATE Update $\pi_{\theta}$ to maximize expected return 
\ENDWHILE
\end{algorithmic}
\end{algorithm}

==> contents/review_comments.tex <==

\section{Comments to resolve}

\subsection{abstract-related}

\red{meta review: it is unclear if the work will be relevant
for realistic scenarios like traffic control. Given other
concerns about the problem setup, the lack of strong
baselines, and questionable experimental setup,}

\red{"However, it is unclear why a continual learning framework was adopted for adapting to different road instances, instead of simply training models for each type of road or perhaps even a single multi-task policy for all scenarios."}
\mengdi{why we use CL is addressed in the intro + also need to address the importance of mixtures }

\red{Finally, this paper does not have any robot applications or even potential robot application that is not a moonshot like smart cities.}
\mengdi{draw connection to mobile robots in the intro}

\subsection{experiments-related}

\red{Moreover, the rotation-equivariant continual RL algorithm is only evaluated in one simulated environment, which leaves a huge question about the potential generalizability of the algorithm.}
\mengdi{Although we use the same simulation platform, we validate the performance of our proposed algorithm in multiple scenarios.}

\mengdi{other environments, what might be the possible group similarities in manipulation tasks}

\red{in application the paper focuses on only one kind of group symmetry, aka rotations. Rotation is arguably
one of the most common group symmetry encountered in robotics, and thus I understand why the authors chose that. However, I am of the opinion that only showing results on rotation is an underdelivery on the promise of RL that leverages group symmetry.}
\mengdi{check whether there exist other group symmetries that can be handled by existing geometric deep learning methods.}

\mengdi{as pointed out by the associate editor, also need to search for strong baselines}


\red{[video]}

\red{The video shows the trained agent in action in different environments, but it does not talk much about the problem setup or the method. From the video, it is not clear why the baseline method suffers so much, which is only clarified in the paper.}
\mengdi{explain the setup with caption in video}

\red{Bad Experimental Setup: In the video it’s clear that in the “lane following task” the car is given goals (i.e. green box) that would have it *not* stay in one lane. This seems indicative of a bad simulated environment that the authors should debug. }
\mengdi{@shiqi: need to double check}




